WoT Store: a Thing and Application Management Ecosystem for the W3C Web of Things

In the next few years, the W3C Web of Things (WoT) platform will represent a reference solution toward the deployment of fully interoperable systems, hence unlocking the potential of the IoT paradigm on several use-cases characterized by the current fragmentation of devices and technologies. At the same time, the worlwide adoption of the W3C WoT architecture depends on many factors, including also the availability of support tools that might facilitate the deployment of novel WoT applications or the integration with traditional IoT systems. To this purpose, the paper presents the WoT Store, a complete software platform enabling the discovery and management of W3C Things, the monitoring of its properties and events, and the invoking of actions, all within the same dashboard. In addition, the platform leverages on the semantic description of each Thing with the goal of easing and automatizing the installation and execution of WoT applications, e.g. defining the behaviour of a Thing or implementing mash-up operations from multiple Things. We sketch the main features, the architecture and the prototypal implementation of the WoT Store. Moreover, we discuss the WoT Store capabilities on three IoT use-cases, i.e. industry 4.0, smart agriculture and home automation.

==> performance.tex <==
\section{Performance Evaluation}
\label{evaluation}

\begin{figure*}[t!]
\centerline{
%\subfigure[\label{sim1}]{\includegraphics[height = 5.0cm,width=6.2cm]{imgs/Time_for_the_emergency_solution_with_40_nodes.pdf}}
%\subfigure[\label{sim2}] {\includegraphics[height = 5.0cm,width=6.2cm]{imgs/Percentage_of_times_the_emergency_is_solved_before_30min_with_40_nodes.pdf}}
%\subfigure[\label{sim3}] {\includegraphics[height =5.0cm, width=6.2cm]{imgs/Number_of_emergency_msgs_sent_over_the_network_with_40_nodes.pdf}}}
\subfigure[\label{sim1}]{\includegraphics[height = 5.0cm,width=6.0cm]{imgs/Time_for_the_emergency_solution_with_40_nodes.pdf}}
\subfigure[\label{sim2}] {\includegraphics[height = 5.0cm,width=6.0cm]{imgs/Percentage_of_times_the_emergency_is_solved_before_30min_with_40_nodes.pdf}}
\subfigure[\label{sim3}] {\includegraphics[height =5.0cm, width=6.0cm]{imgs/Number_of_emergency_msgs_sent_over_the_network_with_40_nodes.pdf}}}
 \caption{The $ERT$, $ERR$ and $EO$ metrics for different values of $\tau$ and $n$=40 are shown in Figures \ref{sim4}, \ref{sim5} and \ref{sim6} respectively. }
\end{figure*}



% \begin{figure*}[!th]
% \centerline{
% \subfigure[\label{exp1}]{\includegraphics[height = 5.0cm,width=6.2cm]{
% imgs/Time_for_the_emergency_solution_with_40_nodes.pdf
% }}
% \subfigure[\label{exp2}] {\includegraphics[height = 5.0cm,width=6.2cm]{imgs/Percentage_of_times_the_emergency_is_solved_before_30min_with_15__of_solvers.pdf}}
% \subfigure[\label{exp3}] {\includegraphics[height =5.0cm, width=6.2cm]{imgs/Percentage_of_times_the_emergency_is_solved_before_30min_with_40_nodes.pdf}}}
% \subfigure[\label{exp3}] {\includegraphics[height =5.0cm, width=6.2cm]{imgs/Time_for_the_emergency_solution_with_15__of_solvers.pdf}}
% \subfigure[\label{exp3}] {\includegraphics[height =5.0cm, width=6.2cm]{imgs/Time_for_the_emergency_solution_with_40_nodes.pdf}}
% \subfigure[\label{exp3}] {\includegraphics[height =5.0cm, width=6.2cm]{imgs/different_percentages.pdf}}
%  \caption{BLA BLA BLA. }
 %\end{figure*}

In this Section, we evaluate the performance of the \textsf{LOCATE} dissemination 
protocol over realistic, simulated emergency scenarios modeled through the \textit{OMNeT++} tool, and compare it against other state-of-art flooding schemes. 
%In particular, w
We rely on the FLORA module \cite{Slabicki18}, which provides a fine-grained modeling of the LoRa PHY layer, and we properly tune the simulation environment with the experimental results presented in Section \ref{experiment_sec} (e.g. range, RSSI and PDR model). 
%In the following, we present the scenario, the competitors, the metrics, and  we finally discuss the simulation results. 
\subsection{Scenario}
We consider a square scenario of $5km$ x $5km$, with $n+1$ LoRa nodes deployed over it. There is exactly one ES, which is assumed stationary and placed at the center of the scenario, while the other $n$ nodes
are randomly distributed over the area, and move according to a Random Direction mobility model, with random speed in range [0.5:3] m/s (typical range of pedestrian mobility). Let $\tau$ represent the percentage of EV over the $n$ nodes available. After a preliminary analysis, we tune the  \textsf{LOCATE} parameters to the following values: $CW_{max}$ (max delay) = 20s, $\gamma$ (stepness) = 0.005, $r$ (communication radius) = 500m. Furthermore, we used the following system parameters: $CW_{min}$ (min delay) = 5s and $\textit{DTN}_{dist}$ (DTN radius) = 50m. We averaged each result over 1000 runs, in order to mitigate the impact of randomness. Each run ends when: (\textit{i}) all the nodes who had received an \texttt{E-REQ} message marked the emergency as solved (i.e. they  received the corresponding \texttt{E-REP}) or (\textit{ii}) the simulated time exceeds a  maximum value, set to 1 day in the following. We neglect the emergency $type$ in this analysis: we assume that the set of $EV$ is pre-decided, and each time an $EV$ receives any \texttt{E-REQ} message, it automatically replies with an \texttt{E-REP} message.
%previously informed about the emergency had marked the emergency as solved Furthermore, we varied the number of nodes $n \in [5, 45]$, while the percentage of solvers, among the entire number of nodes, $l \in [5,30]$ with a step of $5\%$. We ran each simulation 1000 times in order to decrease as much as possible the side effects of all the randomness we need for the scenario configuration. Each simulation has been considered completed in the moment in which all the nodes who previously had been informed about the emergency had marked the emergency as solved, or after one simulated day of running.
\subsection{Other protocols}
We compare our solution against the following multi-hop message dissemination schemes:
\begin{itemize}
\item A \textit{simple flooding strategy}, where nodes  flood the network by re-forwarding the messages they received. Nevertheless, we implement the following improvement for fair comparison: if a node receives an \texttt{E-REQ} message for an emergency already marked as solved (i.e. it has already received the corresponding \texttt{E-REP} message), it avoids to forward the \texttt{E-REQ} and immediately sends back the \texttt{E-REP}. Like the DTN-like state, every node waits for a random timing offset, uniformly distributed between $[0, 20]$ seconds before each retransmission.%devo mettere che anche se ricevo lo stesso identico mesaggio che ho gia' mandato non lo rimando?
\item A \textit{probabilistic scheme}, where the dissemination protocol works identically to the previous case, except that nodes decide to re-transmit a message with probability $q = 40\%$. For fair comparison, the probability is equal to $p_{start}$, i.e. the retransmit probability in the DTN phase used by \textsf{LOCATE} (Equation \ref{eq:dtn_probability}).
\item \textit{\textsf{LOCATE}, basic DTN}, which is our dissemination protocol, without the optimization to the DTN phase in terms of messages sent described in Section \ref{protocol_com}.
\item \textit{\textsf{LOCATE} with 802.11}, which is our dissemination protocol implemented over the popular 802.11 Wi-Fi technology, available on all the existing smartphone devices (assuming the ad-hoc mode is enabled). This is considered as reference for state-of-art phone-based ECS.
\end{itemize}
\subsection{Metrics}
We compute the following network metrics:
\begin{itemize}
\item \textit{Emergency Resolution Time} ($ERT$), defined as the average time which is needed to solve the emergency, and computed as the time interval from when the ES broadcasts the \texttt{E-REQ} message the first time, to when the first corresponding \texttt{E-REP} message is received.
\item \textit{Emergency Resolution Ratio} ($ERR$), defined as the percentage of cases in which the emergency is solved, i.e. the ES receives a \texttt{E-REP} message within a maximum time threshold $E_{thr}$. We set $E_{thr}$ equal to 30 minutes.
\item \textit{Emergency Overhead} ($EO$), defined as the total number of \texttt{E-REQ} messages exchanged among LoRa nodes during the entire simulation. 
\end{itemize}

\begin{figure*}[t!]
\centerline{
%\subfigure[\label{sim4}]{\includegraphics[height = 5.0cm,width=6.2cm]{imgs/Time_for_the_emergency_solution_with_15__of_solvers.pdf}}
%\subfigure[\label{sim5}] {\includegraphics[height = 5.0cm,width=6.2cm]{imgs/Percentage_of_times_the_emergency_is_solved_before_30min_with_15__of_solvers.pdf}}
%\subfigure[\label{sim6}] {\includegraphics[height =5.0cm, width=5.9cm]{imgs/different_percentages.pdf}}}
\subfigure[\label{sim4}]{\includegraphics[height = 4.8cm,width=6.0cm]{imgs/Time_for_the_emergency_solution_with_15__of_solvers.pdf}}
\subfigure[\label{sim5}] {\includegraphics[height = 4.8cm,width=6.0cm]{imgs/Percentage_of_times_the_emergency_is_solved_before_30min_with_15__of_solvers.pdf}}
\subfigure[\label{sim6}] {\includegraphics[height =4.8cm, width=6.0cm]{imgs/different_percentages.pdf}}}
 \caption{The $ERT$, $ERR$ and $EO$ metrics for different values of $n$ and $\tau$=15\% are shown in Figures \ref{sim4}, \ref{sim5} and \ref{sim6} respectively. }
\end{figure*}

\subsection{Results}
In the first analysis, we vary  the ratio of solvers, i.e. $\tau$, on  the x-axis, while keeping fixed the number of nodes, i.e. $n$=40. Figure \ref{sim1} shows the $ERT$ metric for the five schemes described above. It is easy to notice that: (\textit{i}) the performance of all schemes improve when increasing the number of nodes able to send the \texttt{E-REP} message, as expected; (\textit{ii}) the LoRa-based solutions guarantee much lower $ERT$ values than Wi-Fi solutions thanks to the  range expansion; (\textit{iii}) the full \textsf{LOCATE} scheme greatly overcomes the \textit{Flooding} and \textit{Probalistic} schemes, specially in critical scenarios where the number of solvers is low. Figure  \ref{sim2} shows the $ERR$ metric over $\tau$: the \textsf{LOCATE} scheme provides the highest probability of solving the emergency within the  $E_{thr}$ temporal threshold, for all the values of $\tau$. For $\tau$=30\%, the $ERR$ metric approaches the 100\%. 
Figure \ref{sim3} shows the $EO$ metric, and shows that: (\textit{i}) the DTN optimization greatly reduces the number of message sent within the network, and (\textit{ii}) the improvement produced by \textsf{LOCATE} in terms of $ERR$ and $ERT$ does not come at the expense of the $EO$, since the number of messages sent in the network is comparable with the \textit{Probalistic} and \textit{Flooding} schemes.
%ANGELO
%Figure \ref{sim3} reveals that the \textsf{LOCATE} impact the $EO$ index only with very low percentage of solvers, while achieving comparable values with higher number of solvers since the number of messages sent in the network became similar with the other three schemes. 
In the second analysis, we vary the number of nodes, i.e. $n$, while keeping fixed the ratio of solvers, i.e. $\tau$=15\%. We do not show the \textsf{LOCATE} over Wi-Fi, due to the poor performance of the latter. Analogously to Figure \ref{sim1}, Figure \ref{sim4} shows the $ERT$ metric for the four protocols. Increasing $n$ has a positive effect on the $ERT$ metric, since there are more solvers in the neighborhood of the $ES$. However, we can see that the \textsf{LOCATE} scheme provides a considerable delay reduction ($\sim$50\% for $n=5$) even under low density scenarios, which are the most critical for the ECS deployment. Figure \ref{sim5} depicts the $ERR$ metric for the same analysis and confirms the same trend. Finally, Figure \ref{sim6} investigates the impact of the $p_{start}$ parameter of Equation \ref{eq:dtn_probability} on the \textsf{LOCATE} performance. More specifically, we depict the $ERT$ metric on the y-axis, and the $EO$ metric on the y2-axis, for two different configurations of $p_{start}$, i.e. $p_{start}$=40\% and $p_{start}$=80\%. Clearly, for  $p_{start}$=80\%, the probability of retransmitting each message during the DTN phase is higher, and hence also the $EO$ metric increases. However, the interesting result is that the two configurations of $p_{start}$ guarantee almost identical  performance in terms of $ERT$; in other words, the time for solving the emergency is only marginally affected by the probability to retransmit the \texttt{E-REQ} and \texttt{E-REP} messages. For this reason, we used $p_{start}$=40\% in the analysis.


==> protocol.tex <==
\subsection{Dissemination Protocol}
\label{protocol_com}
\begin{figure}
 \centering
 % \includegraphics[width=0.5\textwidth]{imgs/protocol.pdf}
   \includegraphics[scale=0.58]{imgs/protocol.pdf}
  \caption{The \textsc{LOCATE} dissemination protocol for the $i^{th}$-message. State \textit{0} represents the initial state for a node. States \textit{1} and \textit{2} are the states corresponding to the emergency accepting and forwarding. States \textit{3} and \textit{4} are the DTN-based states through which the nodes  keep the emergency alive over the network and possibly spread the solution.}
\label{fig:statechart}
\end{figure}
For easy of disposition, we describe the case where a single emergency is managed within the phone-network, although the \textsf{LOCATE} dissemination scheme is not affected by the presence of multiple $ES$.\\
%In order to show how the dissemination protocol works, let us consider a single emergency in the network for time.
%aggiungere fatto che questa assunzione non e' esagerata visto che ci basta considerare lo stesso protocollo per messaggio
Let $L = \{ l_1, l_2, \dots, l_n\}$ be the set of the $n$ user-owned smartphones equipped with the LoRa radio interface and available within the scenario.
Figure \ref{fig:statechart} depicts the state chart containing all the possible  states and transitions of the node handling the \textit{i-th} emergency.
The protocol works in two main phases: (\textit{i}) a dual, biased contention phase in which nodes become aware of the emergency for the first time, and forward the corresponding \texttt{E-REP} or \texttt{E-REQ} messages, becoming an $EV$ or an $ER$ (based on whether they are able to solve the emergency or not); and (\textit{ii}) a DTN-inspired phase in which each EV implements a store-and-forward mechanism, until receiving an  \texttt{E-REP} message from one of its neighbor.
%and a forwarding phase in which the emergency message keeps being forwarded until someone can solve it. 
The goal of the contention phase is twofold, i.e. to let the possible solvers handle the emergency as soon as possible or, if there are no solvers around, to make the \texttt{E-REQ} cover the longest distance without flooding the network.
%In the first part, after the emergency alert is launched for the first time, we want to let possible solvers handle the emergency as soon as possible or, if there are no solvers around, make the message go as far as possible without flooding the entire network. 
%This is implemented via a biased-contention involving all the 1-hop neighbors of the ES.
%For this reason, there is a contention phase among the surrounding nodes of the emergency source, i.e., the ones inside its transmission range and that share the communication channel. 
%Let $A$ be the acceptance index, such that:
Let $CW_{acc}$ be the acceptance contention window, such that:
%\begin{align}
%	A = D \cdot (1-\frac{1}{e^\frac{s \cdot d(s,j)}{1+\frac{d(s,j)}{r}}}) \label{eq:acceptance_timer}
%\end{align}
\begin{align}
\label{eq:acceptance_timer}
CW_{acc} &= CW_{max} \cdot (1-\frac{1}{e^{\delta}}) \\
\delta &= \gamma \cdot \frac{d(s,j)}{1+\frac{d(s,j)}{r}}
\end{align}
where $CW_{max}$ represents the asymptotic value for the delay, $\gamma$ is a steepness factor, $d(s,j)$ is the distance between the \textit{emergency source} $l_s$ and the $receiver$ node $l_j$, and $r$ is the 
approximated maximum %ANGELO corretto?
%radius of communication
communication radius
(the  parameter is tuned according to the experiments reported in Section \ref{experiment_sec}). When receiving the \texttt{E-REQ} message for the first time, each node starts the \textit{acceptance timer}, which is set to a random value uniformly distributed between $0$ and $CW_{acc}$. It is easy to notice that nodes closer to the \texttt{E-REQ} source will have more chance to win the contention, since they might be able to reach the physical  location of the $ES$ quicker than the other nodes. If the nodes receiving the \texttt{E-REQ} did not send or overhear any \texttt{E-REP} message after a $CW_{max}$ time interval, they start a second contention phase, aimed to detect the best candidate to forward the  \texttt{E-REQ} message.


%Listeners of the emergency first wait for an \textit{acceptance timer}, that is a random value uniformly distributed between $0$ and $CW_{acc}$.
%The more a node is close to the emergency source, the less it has to wait. In fact, the acceptance timer is meant to let closest nodes to quickly solve the emergency if they are able to do it, while making others nodes wait for a possible solution coming from someone else. 
%After this step, if the emergency has not been solved, nodes have to wait for a \textit{forwarding timer}, i.e. 
%a time in which someone could forward the emergency solution before them.
%a timer to avoid collision in forwarding the emergency solution message.
Let $CW_{ft}$ be the forwarding contention window, such that:
\begin{align}
	%FT = D \cdot \frac{1}{e^\frac{s \cdot d(s,j)}{1+\frac{d(s,j)}{r}}} \label{eq:forwarding_timer}
    CW_{ft} = CW_{max} \cdot \frac{1}{e^{\delta}} \label{eq:forwarding_timer}
\end{align}
The value of the \textit{forwarding timer} is random and uniformly distributed between $0$ and $CW_{ft}$. The formulation of the \textit{acceptance timer} (Equation \ref{eq:acceptance_timer}) and of the \textit{forwarder timer} (Equation \ref{eq:forwarding_timer}) is quite similar: however, the goals are opposite, since the  \textit{forwarding timer} gives higher priorities to nodes farther from the \texttt{E-REQ} transmitter, so that the emergency is spread out as fast as possible. 
%On the contrary of the previous case, since we want to make the message go as far as possible, the more the nodes are far, the less they wait for. In this way, the furthest nodes will have more probability to win the contention and will forward the message over the network.
In the second phase of the protocol, after the \textit{forwarding timer}, nodes enter in a DTN-like state till receiving an \texttt{E-REP} message. A node inside the DTN state  regularly broadcasts the \texttt{E-REQ} message by waiting for a random value uniformly distributed between $CW_{min}$ and $CW_{max}$, with $CW_{min} < CW_{max}$.
%emergency to let the rest of the network know about it. In particular, also in this case a node waits for a random value uniformly distributed between $CW_{min}$ and $CW_{max}$, with $CW_{min} < CW_{max}$. 
Since several neighbor nodes can enter the DTN state and keep disseminating the same  information, we adopt some precautions in order to limit the number of messages sent:
\begin{itemize}
\item A node in DTN state forwards a message with a probability equal to $P_{DTN}$, computed as follows:
\begin{align}
	%P = p_{start}^\frac{1}{1+N}
    %P = (p_{start})^\frac{N}{1+N}	%ANGELO dovrebbe essere così, no? più N è grande e meno probabilità di inviare
    P_{DTN} = (p_{start})^\frac{1}{1+N}	%ANGELO rimesso 1... anche se va in contrasto coi punti precedenti... non so, magari bisognerebbe spiegarlo meglio
\label{eq:dtn_probability}
\end{align}
where $p_{start}$ is the initial probability; its impact is analyzed in Section \ref{evaluation}.
%\item Even if it is a random value, the delay in the DTN phase cannot be less than $CW_{min}$ seconds.
\item If a node waiting for its DTN delay overhears an \texttt{E-REQ} message for the same emergency from a neighbor, it reschedules the timer.
\item If a node waiting for its DTN delay overhears more than one \texttt{E-REQ} message for the same emergency from $N$ distinct neighbors, it freezes the retransmission timer, and restarts it after moving of at least $\textit{DTN}_{dist}$ meters.
%specificare cosa si intende per neighbor
\end{itemize}
As soon as a node in DTN state overhears an \texttt{E-REP} message, it starts a \textit{forwarding emergency timer}, i.e., the contention phase previously described, in order to inform the $ES$ as fast as possible. The procedure is started even in case the \texttt{E-REP} message refers to an emergency already marked as solved, in order to increase the chance to reach the $ES$.



%a time in which there is a contention for spreading the solution over the network. Since we need to inform the source of the emergency about the solution as fast as possible, the timer is again a random value uniformly distributed between $0$ and $CW_{acc}$, as defined in Equation \ref{eq:acceptance_timer}. In this way, the more a node is close to the source, the less it has to wait. Hence, it will win the contention and it will be able to spread the solution over the network. 

%The same contention  happens if a node receives an emergency message for en emergency that it has already marked as solved, possibly because a part of the network still needs to be informed about the solution. Instead, if a node just discovers the solution for an emergency previously unknown, it does nothing, since most probably the rest of the network reachable through multi-hop starting from it does not know the emergency. %sistemare

